Buzzard to Cardinal: Improved Mock Catalogs for Large Galaxy Surveys

We present the Cardinal mock galaxy catalogs, a new version of the Buzzard simulation that has been updated to support ongoing and future cosmological surveys, including DES, DESI, and LSST. These catalogs are based on a one-quarter sky simulation populated with galaxies out to a redshift of $z=2.35$ to a depth of $m_{\rm{r}}=27$. Compared to the Buzzard mocks, the Cardinal mocks include an updated subhalo abundance matching (SHAM) model that considers orphan galaxies and includes mass-dependent scatter between galaxy luminosity and halo properties. This model can simultaneously fit galaxy clustering and group--galaxy cross-correlations measured in three different luminosity threshold samples. The Cardinal mocks also feature a new color assignment model that can simultaneously fit color-dependent galaxy clustering in three different luminosity bins. We have developed an algorithm that uses photometric data to improve the color assignment model further and have also developed a novel method to improve small-scale lensing below the ray-tracing resolution. These improvements enable the Cardinal mocks to accurately reproduce the abundance of galaxy clusters and the properties of lens galaxies in the Dark Energy Survey data. As such, these simulations will be a valuable tool for future cosmological analyses based on large sky surveys. The cardinal mock will be released upon publication at https://chunhaoto.com/cardinalsim.

==> addresses.tex <==
\def\kipac{Kavli Institute for Particle Astrophysics and Cosmology, Stanford University, 452 Lomita Mall, Stanford, CA 94035, USA}
\def\slac{Department of Particle Physics and Astrophysics, SLAC National Accelerator Laboratory, 2575 Sand Hill Road, Menlo Park, CA 94025, USA}
\def\stanford{Department of Physics, Stanford University, 382 Via Pueblo, Stanford, CA 94305, USA}

\def\uofa{University of Arizona information}

\def\cpdemail{\tt cpd@stanford.edu}

==> authors.tex <==
\author[To et al.]{
\parbox{\textwidth}{
\Large
Chun-Hao To,$^{1,2,3}$\thanks{Corresponding author: \href{mailto:chto@stanford.edu}{to.87@osu.edu}}
}
\vspace{0.4cm}
\\
\parbox{\textwidth}{
$^{1}$ Center for Cosmology and AstroParticle Physics (CCAPP), Ohio State University, Columbus, OH 43210, USA \\
$^{2}$ Department of Physics, Ohio State University, Columbus, OH 43210, USA \\
$^{3}$ Department of Astronomy, Ohio State University, Columbus, OH 43210, USA
}
}

==> main.tex <==
\AtBeginDocument{\graphicspath{{./}}}\input{4x2pt_N_arxiv_stripped.tex}
